Saying Hello World with VIATRA2 - A Solution to the TTC 2011 Instructive Case

The paper presents a solution of the Hello World! An Instructive Case for the Transformation Tool Contest using the VIATRA2 model transformation tool.

==> eptcsdata.tex <==
\providecommand{\firstpage}{302}
\providecommand{\publicationstatus}{Van Gorp, Mazanek and Rose (Eds.): \\Fifth Transformation Tool Contest (TTC 2011)\\
EPTCS 74, 2011, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.74.25}{10.4204/EPTCS.74.25}}
\pdfoutput=1

